Decentralized Role Assignment in Multi-Agent Teams via Empirical Game-Theoretic Analysis

We propose a method, based on empirical game theory, for a robot operating as part of a team to choose its role within the team without explicitly communicating with team members, by leveraging its knowledge about the team structure. To do this, we formulate the role assignment problem as a dynamic game, and borrow tools from empirical game-theoretic analysis to analyze such games. Based on this game-theoretic formulation, we propose a distributed controller for each robot to dynamically decide on the best role to take. We demonstrate our method in simulations of a collaborative planar manipulation scenario in which each agent chooses from a set of feedback control policies at each instant. The agents can effectively collaborate without communication to manipulate the object while also avoiding collisions using our method.

==> tex/CapturetheFlag.tex <==
\section{Case Study: Capture the Flag}
\label{sec: Case Study}
\subsection{Problem Set-up}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{img/sym.png}
    \caption{An illustration of the symmetric setup of the game.}
    \label{fig:symsetup}
\end{figure}
We experimented our method on a watered-down version of capture-the-flag, where two teams of agents (red and blue) compete to reach the other team's flag. Here, the agents observe the full state, i.e. at any point in time, they know the position of their teammates, their opponents and both flags. We want to predict the role compositions on each team assuming that the agents choose a role before the start of the game and stick to that role throughout the duration of the game. Below, we first describe the environment and roles of interest. Then, we present stylized facts about our prediction on various initial setup of the agent positions and the capabilities of the agents. 

\subsection{Capture-the-flag Environment}
The position of agent $i$ on the field is represented as $\vec{x^{(i)}} = (x^{(i)}, y^{(i)})$. The agents have control over their acceleration in both the x- and y-directions. Denote the control of agent i as $\vec{u}^{(i)}=(u^{(i)}_{x}, u^{(i)}_{y})$. Its movement is then modeled as a double integrator. 
\begin{align*}
\ddot{x}_i &= u^{(i)}_{x}\\
\ddot{y}_i &= u^{(i)}_{y}\\
\end{align*}
We also clip the component-wise velocity of the agents. Let the maximum component-wise velocity of agent $i$ be $v^{(i)}_{max}$. We then require that $\dot{x_i} \in [-v^{(i)}_{max}, v^{(i)}_{max}], \dot{y_i} \in [-v^{(i)}_{max}, v^{(i)}_{max}] \forall i = 1, 2, 3, ..., n$.
To enable interesting offense and defense strategies, we model the collision between two agents on two different teams. When two agents on different teams collide, both agents are sent back to their respective starting point, and have their velocity set to zero. However, we do not model collisions between agents on the same team.

\subsection{Roles Considered}
We consider two roles for the agents in this environment, offense and defense. The goal of the offensive agents is to reach the opponent's flag and thereby seal the victory for its team. The goal of the defensive agent is to prevent the offensive agents on the other team from reaching the defender's own flag, by colliding with the offender. We describe the controls for each role below.
\subsubsection{Offense}
Offensive agents employ a potential-field-based approach with hand-picked weights. They are attracted to the opponent's flag and pushed away from opponents. Specifically, denote the set of opponents for agent $i$ as $\mathcal{OP}(i)$, then the control for agent $i$ is found as
$$\vec{u}^{(i)} = 3\frac{\vec{x}^{(goal)} - \vec{x}^{(i)}}
{||\vec{x}^{(goal)} - \vec{x}^{(i)}||^{2}_{2}} + 0.1
\sum_{j \in \mathcal{OP}(i)}\frac{\vec{x}^{(i)} - \vec{x}^{(j)}}
{||\vec{x}^{(i)} - \vec{x}^{(j)}||^{2}_{2}}$$
\subsubsection{Defense}
The defensive agents take a two-step approach in finding its control. At every time step, the control is found by
\begin{enumerate}
    \item sample an opponent $j$ based on their current distance to the defender's flag
    \item find the control as moving towards the midpoint between the sampled opponent and the defender's own flag $$\vec{u}^{(i)} = (\frac{1}{2}\vec{x}^{(j)} + \frac{1}{2}\vec{x}^{ownflag}) - \vec{x}^{(i)}$$
\end{enumerate}

\subsection{Empirical Game Model}
To construct an empirical game to describe this scenario, we also need to define the payoff structures to all agents. In the case where one team successfully captured the other team's flag, all agents on the winning team receive a positive utility of $+1$ and all the team on the losing team receive $-1$ utility. In the case where the game terminates without one team capturing the other team's flag, all agents on both teams receive $0$ utility.

We make the simplifying assumption that all the agents on one team are symmetric. This assumption allows us to formulate the game as a role-symmetric game with two roles, representing the red and the blue team respectively.

\subsection{Experiment Results}
We ran the experiment for two different cases: symmetric initial condition and asymmetric initial condition. For the symmetric initial conditions, the initial positions of agents on the two teams mirror each other on the field. They also have the same number of players. In the asymmetric initial condition case, we vary the number of agents on the two teams, their starting positions and their maximum component-wise velocities to create asymmetric scenarios. We show that the predicted role compositions match our expectations on both setups.

\subsubsection{Symmetric Initial Condition}

For the symmetric initial conditions, we experimented with two cases, respectively with 3 and 4 players on each team. An illustration of the environment for 3 players is shown in Figure \ref{fig:symsetup}. The role composition prediction for both cases is shown in Table I. As we can see from the composition prediction, for both the 6-player and the 8-player case, the teams favor defense agents heavily. This captures the property of the environment that it is easier for the agents to defend than to attack. The defensive agents need only stay close to its own flag and collide with the opponent when they appear too close. Assuming that all the agents on the other team are defending, there are indeed no incentives for an agent to switch to attacking as that it would be very unlikely to reach the opponent's flag.
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{l|}{Team1} & \multicolumn{2}{l|}{Team2} \\ \cline{2-5} 
                  & Offense      & Defense     & Offense      & Defense     \\ \hline
3v3               & 0.05         & 0.995       & 0.04         & 0.996       \\ \hline
4v4               & 0.112        & 0.878       & 0.112        & 0.878       \\ \hline
\end{tabular}
\label{tab:symnash}
\caption{The Nash equilibria for the symmetric setups. Both teams favor defending significantly over attacking.}
\end{table}


\subsubsection{Asymmetric Initial Condition}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{img/asym.png}
    \caption{Illustration of an asymmetric initial condition of the game.}
    \label{fig:asymsetup}
\end{figure}
For the asymmetric settings, we vary the number of players on each team, their initial positions, and their maximum component-wise velocities. An illustration of the initial positions can be found in Figure \ref{fig:asymsetup}. We present our results in four different cases in Table \ref{tab:asymnash}. 
\begin{itemize}
    \item In the first case, the only aspect different between the two teams are their initial positions in the field. The red team starts closer to the middle of the field than the blue team. This gives the red team a positional advantage in attacking as they are closer to the opponent flag. This is reflected in the role composition prediction, with the red team having a higher percentage of attacking than the blue team.
    \item In case 2, we vary the maximum velocity of the agents on the two teams. This represents the different capabilities in the agents. Note that the only difference between case 1 and case 2 is in the maximum velocity advantage of the blue team in case 2. The prediction reflects this advantage of the blue team as we see the composition of the blue team shifts significantly from its composition in case 1, with a much higher chance to attack.
    \item In case 3, we again go back to letting all agents have the same maximum velocity. However, we vary the number of players. Here, blue team is given an advantage in the number of agents. Even though they still have a positional disadvantage (the same as in case 1), they now have a much more aggressive team composition. In expectation, three out of the four players on the blue team would play offense. This matches our expectation that having more players gives blue team the opportunity to allocate more resources into offense.
    \item Lastly, in case 4, we give the red team both the positional and number advantage. In this case, the predicted composition of the red team is that all the 4 players on the red team would be attacking, whereas all the players on the blue team would be defending. This is again an intuitive result as the red team realizes that their advantage and allocates more resources into attacking.
\end{itemize}


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|ll}
\cline{1-3}
\multicolumn{3}{|c|}{\textbf{Case 1}} & \multicolumn{2}{l}{} \\ \cline{1-3}
 & red & blue &  &  \\ \cline{1-3}
players & 4 & 4 &  &  \\ \cline{1-3}
max\_velocity & 0.75 & 0.75 &  &  \\ \cline{1-3} 
Equilibria & \begin{tabular}[c]{@{}l@{}}31\% attack\\ 69\% defend\end{tabular} & \begin{tabular}[c]{@{}l@{}}15\% attack\\ 85\% defend\end{tabular} &  &  \\ \cline{1-3}
Expected Payoffs & 0.01 & -0.01 &  &  \\ \cline{1-3}
\multicolumn{3}{|c|}{\textbf{Case 2}} &  &  \\ \cline{1-3}
 & red & blue &  &  \\ \cline{1-3}
players & 4 & 4 &  &  \\ \cline{1-3}
max\_velocity & 0.5 & 1.0 &  &  \\ \cline{1-3}
Equilibria & \begin{tabular}[c]{@{}l@{}}13\% attack\\ 87\% defend\end{tabular} & \begin{tabular}[c]{@{}l@{}}60\% attack\\ 40\% defend\end{tabular} &  &  \\ \cline{1-3}
Expected Payoffs & -0.21 & 0.21 &  &  \\ \cline{1-3}
\multicolumn{3}{|c|}{\textbf{Case 3}} &  &  \\ \cline{1-3}
 & red & blue &  &  \\ \cline{1-3}
players & 2 & 4 &  &  \\ \cline{1-3}
max\_velocity & 0.75 & 0.75 &  &  \\ \cline{1-3}
Equilibria & \begin{tabular}[c]{@{}l@{}}29\% attack\\ 71\% defend\end{tabular} & \begin{tabular}[c]{@{}l@{}}68\% attack\\ 32\% defend\end{tabular} &  &  \\ \cline{1-3}
Expected Payoffs & -0.44 & 0.44 &  &  \\ \cline{1-3}
\multicolumn{3}{|c|}{\textbf{Case 4}} &  &  \\ \cline{1-3}
 & red & blue &  &  \\ \cline{1-3}
players & 4 & 2 &  &  \\ \cline{1-3}
max\_velocity & 0.75 & 0.75 &  &  \\ \cline{1-3}
Equilibria & \begin{tabular}[c]{@{}l@{}}100\% attack\\ 0\% defend\end{tabular} & \begin{tabular}[c]{@{}l@{}}0\% attack\\ 100\% defend\end{tabular} &  &  \\ \cline{1-3}
Expected Payoffs & 0.8 & -0.8 &  &  \\ \cline{1-3}
\end{tabular}
\caption{Results for games with asymmetric initial conditions}
\label{tab:asymnash}
\end{table}

\subsection{Discussion}
From the results above, we see that our method produces team composition predictions that match our expectations. Now, we briefly discuss some practical aspects of the method.
\subsubsection{Computation Cost and Symmetry}
The cost of using the EGTA method can be roughly broken down into two parts. The first part of the computation cost comes from simulating different profiles to obtain their corresponding payoffs to construct the empirical game. The second part of the cost comes from solving the equilibria of the empirical game. Although solving for Nash equilibria is believed to be a computationally difficult problem, for a game of a moderate size, our experience shows that replicator dynamics usually converge within a reasonable amount of time (on the scale of 0.1 seconds for a 4 v. 4 setup). Rather, because the number of profiles grows combinatorially with the number of players and strategies, the computation cost is dominated by the simulation cost. In order to address this problem, symmetric assumptions are used to minimize the number of profiles to simulate. For example, in a two-role role-symmetric game with 12 players and 5 strategies, a fully asymmetric formulation results in over 200 million profiles while a role-symmetric formulation requires only 44,100 profiles be simulated. In our case study, the symmetric assumption is a relatively reasonable approximation to the original problem as all the agents on the same team have identical dynamics and payoff structure and their starting positions are relatively close. With the role-symmetric formulation, it takes us around 10 seconds to find the equilibrium for a 4 v. 4 game.
\subsubsection{Generating Meta-Strategies}
In our case study, we used handcrafted controller to describe the two different roles. However, there exist ways of generating controllers when one does not have the domain-specific knowledge required. First, if one has access to trajectory data of human behavior in the environment of interest, one can use imitation learning to generate a set of controllers that resemble the behaviors in the dataset. If one does not have access to past trajectories, one can use policy space response oracle algorithm \cite{tuyls2018generalised} to generate a set of strategies that would likely appear at the equilibrium.

==> tex/symmetry.tex <==
\subsection{Additional Game Theory Preliminaries}
\subsubsection{Symmetric NFG}
A game is \textit{symmetric} if the identity of agents does not matter. As an example, consider rock-paper-scissors. The game is symmetric because rock always wins over scissors, regardless of whether player 1 or player 2 plays rock in this case. Formally, an NFG is symmetric if
\begin{enumerate}
    \item $S^i = S^j = S, \forall i,j \in {1,2,...,|P|}$, i.e. all players share the same strategy set $S=(s_1, s_2, ..., s_{|S|})$
    \item For any permutation matrix $P$ and strategy profile $\vec{s} \in S^{|P|}$, we have $u(P\vec{s}) = Pu(\vec{s})$, i.e. all players have the same incentive structure
\end{enumerate}
For a symmetric NFG with a finite number of players and strategies, we are guaranteed to have a symmetric strategy profile (i.e. every player playing the same mixture) that is a Nash equilibria of the game. On symmetric games, we can define a stronger class of Nash equilibrium called evolutionarily stable strategies (ESS). A symmetric Nash Equilibrium $\vec{\sigma}$ with support $supp(\sigma) \subset S$ is an ESS if either
\begin{itemize}
    \item $|supp(\sigma_i)| = 1$ and $u_i(\vec{\sigma}) > u_i(s, \vec{\sigma}), \forall s \in S^i$, i.e. when $\sigma_i$ is deterministic, then it has to be a strict best response to $\vec{\sigma}_{-i}$, or
    \item $|supp(\sigma_i)| > 1$ and $u_i(\sigma_i, \vec{\sigma'}) > u_i(s, \vec{\sigma'}), \forall s \in S^i, supp(\sigma') \subset supp(\sigma)$, i.e. when $\sigma$ is stochastic, then it has to be a strict best response to every mixed strategy profile with the same support. Here, we used $u_i(s, \vec{\sigma'})$ to denote the payoff of player $i$ playing strategy $s$ while all other agents symmetrically play $\vec{\sigma'}$.
\end{itemize}
The idea of an ESS arises from the study of equilibrium states in evolutionary biology. We note that when the number of agents are sufficiently large, ESS can be safely interpreted, with mild rationality assumptions, as the distribution of the strategies among the population in a steady-state outcome resulted from evolution of the population. We refer interested readers to \cite{nowak2006evolutionary} for a more detailed treatment of the development and interpretation of ESS.

\subsubsection{Role-Symmetric NFG}
We can extend the idea of symmetry to model scenarios where certain a group of players are interchangeable with each other, but not with other agents outside the group. We define a role $R \subset P$ as maximal set of players that are symmetric amongst themselves. Note that a game with $|P|$ roles is fully asymmetric, whereas a game with one role is fully symmetric. Overloading some notations, we formally define a role-symmetric game with $\rho$ roles as a 4-tuple $G=(P, \mathcal{R}, S, u)$, where
\begin{itemize}
    \item $P$ is the set of players
    \item $\mathcal{R} = (R^1, R^2, . . ., R^{\rho})$ is the set of roles. Note that $\mathcal{R}$ is a partition of $P$ as all the players in the game has one and only one role.
    \item $\mathcal{S} = (S^1, S^2, . . ., S^{|P|})$ is a tuple of strategies sets, where $S^i$ denotes the set of strategies of \textit{role} $i$.
    \item $u:  S^{r(1)} \times S^{r(2)} \times . . . \times S^{r(|P|)} \rightarrow \mathcal{R^{|P|}}$ is the joint utility function that maps the strategies chosen by all the agents to their respective payoffs, where $r(\cdot)$ is a mapping from agent index to its role index, i.e. $r(i) = j$ iff $i \in R^j$.
\end{itemize}
The idea of an ESS can be extended to the role-symmetric case, where the conditions above holds true to all the roles, respectively.
